Continuous-Time State Estimation Methods in Robotics: A Survey

Accurate, efficient, and robust state estimation is more important than ever in robotics as the variety of platforms and complexity of tasks continue to grow. Historically, discrete-time filters and smoothers have been the dominant approach, in which the estimated variables are states at discrete sample times. The paradigm of continuous-time state estimation proposes an alternative strategy by estimating variables that express the state as a continuous function of time, which can be evaluated at any query time. Not only can this benefit downstream tasks such as planning and control, but it also significantly increases estimator performance and flexibility, as well as reduces sensor preprocessing and interfacing complexity. Despite this, continuous-time methods remain underutilized, potentially because they are less well-known within robotics. To remedy this, this work presents a unifying formulation of these methods and the most exhaustive literature review to date, systematically categorizing prior work by methodology, application, state variables, historical context, and theoretical contribution to the field. By surveying splines and Gaussian processes together and contextualizing works from other research domains, this work identifies and analyzes open problems in continuous-time state estimation and suggests new research directions.

==> tables/old/nongp_continuous_time.tex <==
% \begin{table*}
%     \centering
%     \resizebox{\textwidth}{!}{
%     \def\arraystretch{1.2}
%     \rowcolors{2}{gray!8}{white}
%     \begin{tabular}{|llllll|}
%         \hline
%          & \textbf{Year} & \textbf{Applications} & \textbf{Estimated Time-Invariant State} & \textbf{Estimated Time-Varying State} & \textbf{Time-Varying State Representation}\\
%          % & \textbf{Year} & \textbf{Applications} & \multicolumn{2}{c}{\textbf{Estimated State}}    & \textbf{Time-Varying State Representation}\\
%          % &               &                       & Time-Invariant & Time-Varying & \\
%         \hline
%         \citet{kim1995ac,kim1995general}* & 1995 & Torque Computation, Animation & - & $\mathbf{r} \in \mathbb{H}_1$ & B\'ezier, Hermite \& B-Spline\\
%         \citet{gortler1995hierarchical}* & 1995 & Theory & - & $\mathbb{R}^n$ & Polynomial and Wavelet \acsp{TBF} \\
%         \citet{anderson1996spline} & 1996 & Bearing-Based Object Tracking & - & ${}^2\mathbf{p}$ & Cubic B-Spline \\
%         \citet{qin1998general}* & 1998 & Theory & - & $\mathbb{R}^n$ & B-Spline\\
%         \citet{jung2001camera} & 2001 & \acs{VIO} & \begin{tabular}{@{}l@{}}-\\ -\end{tabular} & \begin{tabular}{@{}l@{}}$\mathbf{r} \in SO(3)$\\ $\mathbf{p}$\end{tabular} & \begin{tabular}{@{}l@{}}Riemann Summation \\ Spline\end{tabular}\\
%         \citet{ait2009structure} & 2009 & \acs{RS} Object Tracking & $\mathbf{L}$ & $\dot{\mathbf{r}}, \dot{\mathbf{p}}$ & Linear Interpolation \\
%         \citet{bosse2009continuous} & 2009 & \acs{LIDAR} \acs{SLAM} & $\mathcal{M}_S$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation (\& Cubic Spline) \\
%         \citet{klein2009parallel} & 2009 & \acs{RS} \acs{SLAM} & $\mathbf{L} $ & $\mathbf{T} \in SE(3)$ & Riemann Summation \\
%         \citet{bibby2010hybrid} & 2010 & Dynamic \acs{SLAM} & ${}^2\mathcal{M}_O$ & ${}^2\mathbf{T} \in \mathbb{R}^3, \mathbf{D}$ & Non-Uniform Cubic Splines \\
%         \citet{forssen2010rectifying} & 2010 & \acs{RSC} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{hadzagic2011bayesian} & 2011 & Object Tracking & - & ${}^2\mathbf{p}$ & Non-Uniform Cubic B-Spline \\
%         \citet{ringaby2011scan} & 2011 & \acs{RSC} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{fleps2011optimization} & 2011 & Visual-Inertial Calibration & $\mathbf{b}_g, \mathbf{b}_a, \mathbf{T}_E, \mathbf{g}, \dot{\mathbf{p}}_\text{scale}$ & $\mathbf{p} \in \mathbb{R}^3, \mathbf{r} \in \mathbb{R}^4$ & Cubic B-Splines \\
%         \citet{karpenko2011digital} & 2011 & \acs{RSC} for Video Stabilization & $\mathbf{K}$ & $\mathbf{r} \in SO(3)$ & Linear Interpolation \\
%         \citet{hedborg2012rolling} & 2012 & \acs{RSC} for \acs{SFM} & $\mathbf{L}$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{bosse2012zebedee} & 2012 & \acs{LIDAR}-Inertial \acs{SLAM} & $\mathbf{b}_g, \mathbf{b}_a, \mathbf{t}_E, \mathcal{M}_S$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{jia2012probabilistic} & 2012 & \acs{RSC} for Video Rectification & - & $\mathbf{r} \in SO(3)$ & Linear Interpolation \\
%         \citet{furgale2012continuous,furgale2015continuous}* & 2012/2015 & \begin{tabular}{@{}l@{}}Theory\\ Visual-Inertial Calibration\\ \acs{RS} Localization\end{tabular} & \begin{tabular}{@{}l@{}}-\\$\mathbf{T}_E, \mathbf{g}, \mathbf{L}$ \\-\end{tabular} & \begin{tabular}{@{}l@{}}$\mathbb{R}^n$\\ $\mathbf{r} \in \mathbb{R}^3 \text{(\acs{CGR})}, \mathbf{p}, \mathbf{b}_g, \mathbf{b}_a$\\$\mathbf{r} \in \mathbb{R}^3 \text{(\acs{CGR})}, \mathbf{p}$\end{tabular} & \begin{tabular}{@{}l@{}}\acsp{TBF}\\ B-Splines\\ B-Splines\end{tabular} \\
%         \citet{furgale2013unified} & 2013 & Visual-Inertial Calibration & $\mathbf{T}_E, \mathbf{t}_E, \mathbf{g}$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in \mathbb{R}^6 \text{(\acs{CGR})}$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}\acsp{TBF} / Quintic B-Spline\\\acsp{TBF} / Cubic B-Splines\end{tabular} \\
%         \citet{lovegrove2013spline}* & 2013 & \begin{tabular}{@{}l@{}}\acs{RS} \acs{SLAM}\\\acs{RS}-Inertial \acs{SLAAM}\end{tabular} & \begin{tabular}{@{}l@{}}$\bm{\rho}_d$\\ $\mathbf{b}_g, \mathbf{b}_a, \mathbf{K}, \mathbf{T}_E, \mathbf{g}, \bm{\rho}_d$\end{tabular} & $\mathbf{T} \in SE(3)$ & Cubic B-Spline \\
%         \citet{anderson2013towards,anderson2015relative} & 2013/2015 & \acs{LIDAR} \acs{SLAM} & $\mathbf{L}$ & \begin{tabular}{@{}l@{}}$\dot{\mathbf{T}}$\\$\mathbf{T} \in SE(3)$\end{tabular} & \begin{tabular}{@{}l@{}}\acsp{TBF} / Cubic B-Spline\\Riemann Summation\end{tabular} \\
%         \citet{anderson2013ransac} & 2013 & \acs{LO} & - & \begin{tabular}{@{}l@{}}$\dot{\mathbf{T}}$\\ $\mathbf{T} \in SE(3)$\end{tabular} & \begin{tabular}{@{}l@{}}Feature Tracking + RANSAC\\ Riemann Summation\end{tabular} \\
%         \citet{dong2013lighting} & 2013 & \acs{PC} \acs{MDC} for \acs{PC} Registration for \acs{LO} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{oth2013rolling} & 2013 & \acs{RS} Calibration & $t_\text{RS}$ & $\mathbf{r} \in \mathbb{R}^3, \mathbf{p} \in \mathbb{R}^3$ & \acsp{TBF} / Uniform Cubic B-Spline \\
%         \citet{li2013real} & 2013 & \acs{VIO} & - & \begin{tabular}{@{}l@{}}$\mathbf{r} \in SO(3)$\\ $\mathbf{p}, \dot{\mathbf{p}}$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Euler Method (\acs{RK})\\ Trapezoidal Rule (\acs{RK})\\ Discrete-Time Values\end{tabular} \\
%         \citet{sheehan2013continuous} & 2013 & \acs{LIDAR} Localization & - & $\mathbf{T} \in \mathbb{R}^6 \text{(\acs{RPY})}$ & Cubic Catmull-Rom Spline \\
%         \citet{zlot2013efficient,zlot2014efficient} & 2013/2014 & \acs{LIDAR}-Inertial Odometry & $\mathcal{M}_S$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Uniform Linear / Cubic B-Spline \\
%         \citet{rehder2014spatio} & 2014 & \acs{LIDAR}-Visual-Inertial Calibration & $\mathbf{T}_E, \mathbf{T}_E, \mathbf{g}$ & $\mathbf{T} \in \mathbb{R}^6 \text{(\acs{CGR})}, \mathbf{b}_g, \mathbf{b}_a$ & \acsp{TBF} / Quintic B-Splines \\
%         \citet{alismail2014continuous} & 2014 & \acs{PC} \acs{MDC} for \acs{PC} Registration for \acs{LO} & - & $\mathbf{T} \in \mathbb{R}^6 \text{(\acs{CGR})}$ & Uniform Linear to Quintic B-Spline \\
%         \citet{zhang2014loam,zhang2017low} & 2014/2017 & \acs{PC} \acs{MDC} for \acs{PC} Registration for \acs{LO} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{anderson2014hierarchical} & 2014 & \acs{TE} & - & $\mathbf{T} \in \mathbb{R}^6$ & Polynomial and Wavelet \acsp{TBF} \\
%         \citet{patron2015spline} & 2015 & \begin{tabular}{@{}l@{}}\acs{RS} \acs{SLAM}\\\acs{RS}-Inertial \acs{SLAAM}\end{tabular} & \begin{tabular}{@{}l@{}}$\bm{\rho}_d$\\ $\mathbf{b}_g, \mathbf{b}_a, \mathbf{K}, \mathbf{T}_E, \mathbf{g}, \bm{\rho}_d$\end{tabular} & $\mathbf{T} \in SE(3)$ & Cubic B-Spline \\
%         \citet{kerl2015dense} & 2015 & \acs{RS} \acs{RGBD} Odometry & - & $\mathbf{T} \in SE(3)$ & Uniform Cubic B-Spline \\
%         \citet{mueggler2015continuous} & 2015 & Event Camera Localization & - & $\mathbf{T} \in SE(3)$ & Uniform Cubic B-Spline \\
%         \citet{dube2016non} & 2016 & \acs{LIDAR}-Inertial-Wheeled \acs{SLAM} & $\mathcal{M}_S$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Splines \\
%         \multirow{3}{*}{\citet{rehder2016general}} & \multirow{3}{*}{2016} & Extrinsic Calibration Theory & $\mathbf{t}_E$ & - & \acsp{TBF}\\ & & \acs{LIDAR}-Visual-Inertial Calibration & $b_r, \mathbf{T}_E, \mathbf{t}_E, \mathbf{g}, \mathbf{L}_\pi$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in \mathbb{R}^6 \text{(\acs{AA})}$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Quintic B-Splines\\ Cubic B-Splines\end{tabular} \\
%         \citet{rehder2016extending} & 2016 & Multi-\acs{IMU} Visual-Inertial Calibration & $\mathbf{S}_g, \mathbf{M}_g, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{T}_E, \mathbf{t}_E, \mathbf{g}$ & \begin{tabular}{@{}l@{}}$(\mathbf{T} \in \mathbb{R}^6 \text{(\acs{AA})})^N$\\ $(\mathbf{b}_g\mathbf{b}_a)^N$\end{tabular} & \begin{tabular}{@{}l@{}}Quintic B-Splines\\ Cubic B-Splines\end{tabular} \\
%         \citet{kim2016direct} & 2016 & \acs{RS} \acs{SLAM} & $\mathbf{p}_d$ & $\mathbf{T} \in SE(3)$ & Cubic B-Spline \\
%         \citet{sommer2016continuous}* & 2016 & \begin{tabular}{@{}l@{}}Theory\\ Attitude Estimation\end{tabular} & - & \begin{tabular}{@{}l@{}}$\mathcal{L}$\\ $\mathbf{r} \in \mathbb{H}_1$\end{tabular} & B-Spline \\
%         % \citet{rehder2017camera} & 2017 & Visual-Inertial Calibration & $t_e, \bm{r}_C \in \mathbb{R}, \mathbf{S}_g, \mathbf{M}_g, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{p}_{ia}, \mathbf{r}_{ga}, \mathbf{T}_E, \mathbf{t}_E, \mathbf{g}, \mathbf{m}_o \in \mathbb{R}^7$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in \mathbb{R}^6 \text{(AA)}$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Uniform Quintic B-Spline\\ Uniform Cubic B-Spline\end{tabular} \\
%         \citet{rehder2017camera} & 2017 & Visual-Inertial Calibration & $t_e, \bm{r}_C, \mathbf{S}_g, \mathbf{M}_g, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{p}_{ia}, \mathbf{r}_{ga}, \mathbf{T}_E, \mathbf{t}_E, \mathbf{g}, \mathbf{m}_o$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in \mathbb{R}^6 \text{(AA)}$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Uniform Quintic B-Spline\\ Uniform Cubic B-Spline\end{tabular} \\
%         \citet{droeschel2017continuous} & 2017 & \acs{PC} \acs{MDC} for \acs{LIDAR} \acs{SLAM} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{vandeportaele2017pose} & 2017 & \acs{RS} Localization & - & $\mathbf{T} \in SE(3)$ & Uniform Cubic B-Spline \\
%         \citet{li2016fitting,li2017track,li2018joint} & 2017/2018 & Bearing-based Tracking & - & ${}^2\mathbf{p}$ & Polynomial and Sinusoidal \acsp{TBF} \\
%         \citet{droeschel2018efficient} & 2018 & \acs{PC} \acs{MDC}, \acs{LIDAR} \acs{SLAM} & $\mathcal{M}_S$ & $\mathbf{T} \in SE(3)$ & Cubic B-Spline \\
%         \citet{lowe2018complementary} & 2018 & \acs{LIDAR}-Visual-Inertial \acs{SLAM} & $\mathbf{S_3}$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Uniform Linear Spline \\
%         \citet{mueggler2018continuous} & 2018 & Event-Inertial Localization & $\mathbf{b}_g, \mathbf{b}_a, \mathbf{r}_\mathbf{g} \in \mathbb{R}^2$ & $\mathbf{T} \in SE(3)$ & Uniform Cubic B-Spline \\
%         \citet{park2018elastic} & 2018 & \acs{LIDAR}-Inertial \acs{SLAM} & $\mathbf{b}_g, \mathbf{b}_a, \mathcal{M}_S$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{ovren2018spline} & 2018 & \acs{RS} Visual-Inertial \acs{SLAM} & $\bm{\rho}_d$ & $\mathbf{T} \in \mathbb{H}_1 \times \mathbb{R}^3$ & Cubic B-Splines \\
%         \citet{ovren2019trajectory} & 2019 & \acs{RS} Visual-Inertial \acs{SLAM} & $\bm{\rho}_d$ & $\mathbf{T} \in \mathbb{H}_1 \times \mathbb{R}^3, SE(3)$ & Cubic B-Spline(s) \\
%         \citet{sommer2020efficient}* & 2020 & \begin{tabular}{@{}l@{}}Theory\\ \acs{TE}\\ Visual-Inertial Calibration\end{tabular} & \begin{tabular}{@{}l@{}}-\\ -\\$\mathbf{b}_g, \mathbf{b}_a, \mathbf{T}_E, \mathbf{g}$\end{tabular} & \begin{tabular}{@{}l@{}}$\mathcal{L}$\\ $\mathbf{T} \in SO(3) \times \mathbb{R}^3, SE(3)$\\ $\mathbf{T} \in SO(3) \times \mathbb{R}^3, SE(3)$\end{tabular} & \begin{tabular}{@{}l@{}}B-Spline\\Cubic to Quintic B-Spline(s)\\Quartic Uniform B-Spline(s)\end{tabular} \\
%         \citet{pacholska2020relax} & 2020 & Certifiable Range-Based Localization & - & ${}^n\mathbf{p}$ & Polynomial and Sinusoidal \acsp{TBF}\\
%         \citet{shan2020lio} & 2020 & \acs{PC} \acs{MDC} for \acs{LIDAR}-Inertial \acs{SLAM} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\ 
%         \citet{lv2020targetless} & 2020 & \acs{LIDAR}-Inertial Calibration & $\mathbf{b}_g, \mathbf{b}_a, \mathbf{T}_E$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Uniform Cubic B-Spline \\
%         \citet{hug2020hyperslam} & 2020 & Visual-Inertial \acs{SLAM} & $\mathbf{b}_g, \mathbf{b}_a, \mathbf{g}, \mathbf{L}$ & $\mathbf{T} \in \mathbb{H}_1 \times \mathbb{R}^3$ & Cubic B-Spline(s) \\
%         \citet{park2020spatiotemporal} & 2020 & \acs{LIDAR}-Visual Calibration & $\mathbf{T}_E, \mathbf{t}_E$ & $\mathbf{T} \in SE(3)$ & Linear Interpolation \\
%         \citet{park2021elasticity} & 2021 & \acs{LIDAR}-Visual-Inertial \acs{SLAM} & $\mathbf{b}_g, \mathbf{b}_a, \mathbf{t}_E, \mathcal{M}_S$ & $\mathbf{T} \in SE(3) \text{ / } SO(3) \times \mathbb{R}^3$ & Linear Interpolation / Uniform Cubic B-Spline \\
%         \citet{shan2021lvi} & 2021 & \acs{PC} \acs{MDC} for \acs{LIDAR}-Visual-Inertial \acs{SLAM} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\ 
%         \citet{lv2021clins} & 2021 & \begin{tabular}{@{}l@{}}\acs{PC} \acs{MDC}\\ \acs{LIO}\end{tabular} & \begin{tabular}{@{}l@{}} -\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3, \dot{\mathbf{p}} \text{ \& } \mathbf{T} \in SO(3) \times \mathbb{R}^3$\\ $\mathbf{T} \in SO(3) \times \mathbb{R}^3$\end{tabular} & \begin{tabular}{@{}l@{}}Riemann Summation \& Uniform B-Splines\\ Uniform B-Splines\end{tabular} \\
%         \citet{yang2021asynchronous} & 2021 & Multi-Camera \acs{SLAM} & $\mathbf{L}$ & $\mathbf{T} \in SE(3)$ & Non-Uniform Cubic B-Spline \\
%         \citet{quenzel2021real} & 2021 & Surfel Registration for \acs{LO} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Non-Uniform Quadratic B-Splines \\
%         \citet{xu2021fast} & 2021 & \acs{LIO} \& \acs{PC} \acs{MDC} & $\mathbf{g}$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3, \dot{\mathbf{p}}$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Forward/Backward Riemann Summation\\ Discrete-Time Values\end{tabular} \\
%         \citet{xu2022fast} & 2022 & \acs{LIO} \& \acs{PC} \acs{MDC} & $\mathbf{g}$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3, \dot{\mathbf{p}}$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Constant-Acceleration Integration %Forward/Backward Constant-Acceleration Integration
%         \\ Discrete-Time Values\end{tabular} \\
%         \citet{ramezani2022wildcat} & 2022 & \acs{LIDAR}-Inertial \acs{SLAM} & $\mathbf{b}_g, \mathbf{b}_a, \mathcal{M}_S$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation, Cubic B-Spline \\
%         \citet{dellenbach2022ct} & 2022 & \acs{PC} \acs{MDC} for \acs{PC} Registration for \acs{LO} & - & $\mathbf{T} \in SO(3) \times \mathbb{R}^3$ & Linear Interpolation \\
%         \citet{cioffi2022continuous} & 2022 & Visual-Inertial-\acs{GNSS} \acs{SLAM} & $\mathbf{T}_E, \mathbf{t}_E, \mathbf{g}, \mathbf{L}$ & $\mathbf{T} \in SO(3) \times \mathbb{R}^3, \mathbf{b}_g, \mathbf{b}_a$ & Cubic to Sextic Uniform B-Splines \\
%         \citet{hug2022continuous} & 2022 & Stereo Visual-Inertial \acs{SLAM} & $\mathbf{g}, \mathbf{L}$ & $\mathbf{T} \in \mathbb{H}_1 \times \mathbb{R}^3, \mathbf{b}_g, \mathbf{b}_a$ & Uniform Cubic B-Splines \\
%         \citet{tirado2022jacobian}* & 2022 & \begin{tabular}{@{}l@{}}Theory\\ Object Tracking\end{tabular} & - & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SE(3)$\\ $\mathbf{D} \in (SE(3))^D$\end{tabular} & \begin{tabular}{@{}l@{}}Non-Uniform B-Spline\\ Non-Uniform Cubic B-Spline\end{tabular} \\
%         \citet{mo2022continuous} & 2022 & Visual-Inertial \acs{SLAM} & $\mathbf{K}, \mathbf{r}_\mathbf{g} \in \mathbb{R}^2, s, \bm{\rho}_d$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3$\\ $\bm{r}_C \in \mathbb{R}^2, \mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Cubic Splines\\ Discrete-Time Values\end{tabular} \\
%         \citet{huai2022continuous} & 2022 & \acs{RS} Visual-Inertial Calibration & $t_{\text{\acs{RS}}}, \{\mathbf{S}_g, \mathbf{M}_g, \mathbf{r}_{ga}\} \in \mathbb{R}^{3 \times 3}, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{T}_E, \mathbf{t}_E, \mathbf{r}_\mathbf{g}$ & $\mathbf{T} \in \mathbb{R}^6 \text{(AA)}, \mathbf{b}_g, \mathbf{b}_a$ & Uniform Quintic B-Splines \\
%         \citet{wang2022visual} & 2023 & Event-Based \acs{VO} & - & ${}^2\mathbf{p}$ & B-Spline \\
%         \citet{lang2022ctrl} & 2022 & Visual-Inertial \acs{SLAM} & $t_{\text{\acs{RS}}}, \bm{\rho}_d$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Uniform Cubic B-Splines\\ Discrete-Time Values\end{tabular} \\
%         \citet{lv2022observability} & 2022 & \acs{LIDAR}-Inertial Calibration & $b_r, s_r, \mathbf{m}_r \in \mathbb{R}^4, \mathbf{S}_g, \mathbf{M}_g, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{T}_E, \mathbf{t_E}, \mathbf{g}$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Uniform Cubic B-Splines\\ Discrete-Time Values\end{tabular} \\
%         \citet{lv2023continuous} & 2023 & \acs{LIDAR}-Visual-Inertial \acs{SLAM} & $\mathbf{t}_E, \bm{\rho}_d$ & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Uniform Cubic B-Splines\\ Discrete-Time Values\end{tabular} \\
%         \citet{lang2023coco} & 2023 & \acs{LVIO} & - & \begin{tabular}{@{}l@{}}$\mathbf{T} \in SO(3) \times \mathbb{R}^3$\\ $\mathbf{b}_g, \mathbf{b}_a$\end{tabular} & \begin{tabular}{@{}l@{}}Non-Uniform Cubic B-Splines\\ Discrete-Time Values\end{tabular} \\
%         \citet{nguyen2023slict} & 2023 & \acs{PC} \acs{MDC} for \acs{LIDAR}-Inertial \acs{SLAM} & - & $\mathbf{r} \in SO(3), \mathbf{p}, \dot{\mathbf{p}}, \mathbf{b}_g, \mathbf{b}_a$ & Linear Interpolation \\
%         \citet{zheng2023ectlo} & 2023 & \acs{LO} & - & $\mathbf{T} \in SE(3)$ & Linear Interpolation \\
%         \citet{chen2023direct} & 2023 & \acs{PC} \acs{MDC} for \acs{LIO} & - & $\mathbf{T} \in \mathbb{H}_1 \times \mathbb{R}^3, \dot{\mathbf{p}}, \mathbf{b}_g, \mathbf{b}_a$ & Constant-Jerk Integration \\
%         \citet{li2023continuous}* & 2023 & Theory, \acs{UWB}-Inertial Localization & $\mathbf{T}_E, \mathbf{r}_\mathbf{g}$ & $\mathbf{T} \in \mathbb{H}_1 \times \mathbb{R}^3, \mathbf{b}_g, \mathbf{b}_a$ & Uniform Cubic B-Splines \\
%         \citet{zheng2024trajlo} & 2024 & \acs{LO} & - & $\mathbf{T} \in SE(3)$ & Linear Interpolation \\
%         \citet{nguyen2024eigen} & 2024 & \acs{LIO} & - & \begin{tabular}{@{}l@{}} $\mathbf{r} \in SO(3), \mathbf{p}$ \\ 
%         $\mathbf{b}_g, \mathbf{b}_a$ \end{tabular} & \begin{tabular}{@{}l@{}} Uniform Cubic B-Splines \\ Discrete-Time Values \end{tabular} \\
%         \citet{lv2024cta} & 2024 & \acs{LO} & - & $\mathbf{r} \in SO(3), \mathbf{p}$ & Uniform Cubic B-Splines \\
%         \hline
%     \end{tabular}
%     }
%     \vspace{1mm}
%     \caption{Linear interpolation, numerical integration and temporal basis \ac{CT} state representation works. Asterisks (*) indicate works that significantly expanded the mathematical formulation of \acsp{TBF} and splines. See \cref{tab:variable_definitions} for definitions.}
%     \label{tab:nongp_ct_applications_robotics}
% \end{table*}

% % \footnotesize{$^{1}$ $t_e, \bm{r}_C \in \mathbb{R}, \mathbf{S}_g, \mathbf{M}_g, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{p}_{ia}, \mathbf{r}_{ga}, \mathbf{T}_E, \mathbf{t}_E, \mathbf{g}, \mathbf{m}_o \in \mathbb{R}^7$}
% % \footnotesize{$^{2}$ $t_{\text{\acs{RS}}}, \{\mathbf{S}_g, \mathbf{M}_g, \mathbf{r}_{ga}\} \in \mathbb{R}^{3 \times 3}, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{T}_E, \mathbf{t}_E, \mathbf{r}_\mathbf{g}$}
% % \footnotesize{$^3$ $b_r, s_r, \mathbf{m}_r \in \mathbb{R}^4, \mathbf{S}_g, \mathbf{M}_g, \mathbf{G}_g, \mathbf{S}_a, \mathbf{M}_a, \mathbf{T}_E, \mathbf{t_E}, \mathbf{g}$}

==> tables/old/spline_analytic_derivatives.tex <==
\begin{table}[ht]
    \centering
    \caption{Works providing analytic Jacobians for Lie group splines and their temporal derivatives. $\mathcal{L}$ denotes any Lie group.}
    \vspace{-3mm}
    \resizebox{\linewidth}{!}{
    % \def\arraystretch{1.2}
    \rowcolors{2}{gray!8}{white}
    \begin{tabular}{|l|lll|}
        \hline
         \textbf{Lie Group} & \textbf{Spline (\nth{0} Derivative)} & \textbf{\nth{1} Derivative} & \textbf{\nth{2} Derivative} \\
        \hline
        % $\mathbb{R}^3$$^*$ & \cite{li2023continuous} &  & \cite{li2023continuous} \\
        $SO(3)$ & \cite{sommer2020efficient} & \cite{sommer2020efficient} & \cite{sommer2020efficient} \\
        $SE(3)$ & \cite{tirado2022jacobian} & \cite{tirado2022jacobian} & - \\
        $SU(2)$ & \cite{li2023continuous} & \cite{li2023continuous} & - \\
        $\mathcal{L}$ & \cite{johnson2024continuous} & \cite{johnson2024continuous} & \cite{johnson2024continuous} \\
        \hline
    \end{tabular}
    }
    \label{tab:splines_lie_groups_analytic_jacobians}
\end{table}

==> visual_toc.tex <==
\begin{figure*}[ht]
    \centering
    % \fbox{\includegraphics[width=\linewidth]{figures/ct_survey_toc.pdf}}
    \includegraphics[width=\linewidth]{figures/ct_survey_toc.pdf}
    \put(-0.68\linewidth,385){\Large{\hyperref[sec:state_estimation_in_robotics]{II. State Estimation in Robotics}}}
    \put(-0.84\linewidth,258){\normalsize{\hyperref[sec:state_estimation_in_robotics:preliminaries]{II. \textit{A.} Preliminaries}}}
    \put(-0.5\linewidth,258){\normalsize{\hyperref[sec:state_estimation_in_robotics:discrete_time_state_estimation]{II. \textit{B.} \acf{DT}} vs. \hyperref[sec:state_estimation_in_robotics:continuous_time_state_estimation]{II. \textit{C.} \acf{CT}}}}
    \put(-0.94\linewidth,231){\normalsize{\textbf{Interpolation \& Integration}}}
    \put(-0.96\linewidth,145){\normalsize{\hyperref[sec:theory:interpolation_and_integration]{III. \textit{A.} Theory} \& \hyperref[sec:survey:interpolation_and_integration]{IV. \textit{A.} Survey}}}
    \put(-0.58\linewidth,231){\normalsize{\textbf{Temporal Splines}}}
    \put(-0.62\linewidth,145){\normalsize{\hyperref[sec:theory:temporal_splines]{III. \textit{B.} Theory} \& \hyperref[sec:survey:temporal_splines]{IV. \textit{B.} Survey}}}
    \put(-0.29\linewidth,231){\normalsize{\textbf{\aclp{TGP}}}}
    \put(-0.29\linewidth,145){\normalsize{\hyperref[sec:theory:temporal_gaussian_processes]{III. \textit{C.} Theory} \& \hyperref[sec:survey:temporal_gaussian_processes]{IV. \textit{C.} Survey}}}
    \put(-0.63\linewidth,115){\Large{\hyperref[sec:open_problems]{V. Open Problems}}}
    \put(-0.74\linewidth,100){\normalsize{\hyperref[sec:open_problems:temporal_splines]{V. \textit{A.} Temporal Splines}}}
    \put(-0.48\linewidth,100){\normalsize{\hyperref[sec:open_problems:temporal_gaussian_processes]{V. \textit{B.} \aclp{TGP}}}}
    \put(-0.66\linewidth,88){\small{Knot Selection}}
    \put(-0.53\linewidth,88){\small{$\longleftrightarrow$}}
    \put(-0.48\linewidth,88){\small{State Time Selection}}
    \put(-0.82\linewidth,77){\small{Certifiability \& Recovery Guarantees}}
    \put(-0.53\linewidth,77){\small{$\longleftrightarrow$}}
    \put(-0.48\linewidth,77){\small{Certifiability \& Recovery Guarantees}}
    % \put(-0.64\linewidth,66){\small{$\vdots$}}
    % \put(-0.38\linewidth,66){\small{$\vdots$}}
    \put(-0.735\linewidth,66){\small{Incremental Optimization}}
    \put(-0.48\linewidth,66){\small{Complex Process Models}}
    \put(-0.645\linewidth,55){\small{Initialization}}
    \put(-0.73\linewidth,44){\small{Covariance Interpolation}}
    \put(-0.69\linewidth,20){\Large{\hyperref[sec:applications_to_other_domains]{VI. Applications to Other Domains}}}
    \put(-0.75\linewidth,5){\normalsize{\hyperref[sec:applications_to_other_domains:temporal_splines]{VI. \textit{A.} Temporal Splines}}}
    \put(-0.48\linewidth,5){\normalsize{\hyperref[sec:applications_to_other_domains:temporal_gaussian_processes]{VI. \textit{B.} \aclp{TGP}}}}
    \caption{Visual Table of Contents.}
    \label{fig:visual_toc}
\end{figure*}
